Identifying Correlation Clusters in Many-Body Localized Systems

We introduce techniques for analysing the structure of quantum states of many-body localized (MBL) spin chains by identifying correlation clusters from pairwise correlations. These techniques proceed by interpreting pairwise correlations in the state as a weighted graph, which we analyse using an established graph theoretic clustering algorithm. We validate our approach by studying the eigenstates of a disordered XXZ spin chain across the MBL to ergodic transition, as well as the non-equilibrium dyanmics in the MBL phase following a global quantum quench. We successfully reproduce theoretical predictions about the MBL transition obtained from renormalization group schemes. Furthermore, we identify a clear signature of many-body dynamics analogous to the logarithmic growth of entanglement. The techniques that we introduce are computationally inexpensive and in combination with matrix product state methods allow for the study of large scale localized systems. Moreover, the correlation functions we use are directly accessible in a range of experimental settings including cold atoms.

==> rescaling_entanglement.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{./figures/rescaling_coeff_page0.6.pdf}
	\caption{
	 Scaling collapse of the average number of clusters $n$ divided by system size as a function of the disorder obtained using our modified Girvan-Newman approach. For the collapse, the disorder strength was rescaled to take the form $(W-W_c)/L^u$ with $W_c=3.8$ and $u=1.26$. An eigenstate with bipartite entanglement entropy in the middle of the chain bigger than $0.6$ times the page value was considered to be ergodic and therefore was counted as one cluster, idepedently of the result of the graph theory approach. Inset: average number of clusters $n$ divided by system size as a function of disorder strength $W$.}
	\label{fig:collapse}
	%produced with /space/ge72viw/dmrgx_mbl_data/F_mod_plus_entropy.py
\end{figure}
We note that if the system is ergodic, then we would expect the mutual information to be uniform on average between all pairs of sites \cite{Giusepe_mutual_info_mbl}. 
%
In this case, the optimal clustering is a single cluster containing all sites. 
%
For this reason, when the half chain entanglement entropy is greater than a significant fraction $\alpha$ of the Page value~\cite{Page1993} (in practice $\alpha=60\%$), we bypass our algorithm and select the whole system as a cluster. 
%
In this case, the modularity has low value for all possible decompositions ($\lessapprox 0.3$), which indicates that no good clustering structure is to be found according to graph theory \cite{invention_modularity,first_girvan_newman}. We show in appendix \ref{sec:thresholds} than the choice of $\alpha$ does change significantly the results
%
After focussing on the average cluster size, we will now investigate the structure of individual eigenstates using the clustering algorithms. 


==> rescaling_modularity.tex <==
\begin{figure}[t]
	\includegraphics[width=\columnwidth]{./figures/tsmirescaling_global_coeff0.3.pdf}
	\caption{
	 Scaling collapse of the average number of clusters $n$ divided by system size as a function of the disorder obtained using our modified Girvan-Newman approach. For the collapse, the disorder strength was rescaled to take the form $(W-W_c)/L^u$ with $W_c=3.8$ and $u=1.26$. When the modularity was lower than $0.3 \times(1-a_{W=6}/L)$, the state was considered as fully ergodic and made of only one cluster. The coefficient $a_{W=6}$ has been fitted to take into account the finite size effects at $W=6$, according to the finite size scaling: $Q_L=q-\frac{a}{L}$ of the average modularity $Q_L$ obtained for system size L. Inset: average number of clusters $n$ divided by system size as a function of disorder strength $W$.}
	\label{fig:collapse}
	%produced with /space/ge72viw/dmrgx_mbl_data/F_mod_plus_entropy.py
\end{figure}
We note that if the system is ergodic, then we would expect the mutual information to be uniform on average between all pairs of sites \cite{Giusepe_mutual_info_mbl}. 
%
In this case, the optimal clustering is a single cluster containing all sites. 
%
For this reason, when the maximum modularity obtained through the course of our algorithm is too low, we select the whole system as one cluster.
%
Since for equivalent cluster structures, the value of the modularity increases with system size (see appendix \ref{sec:scaling modularity}), we need to choose a different modularity threshold $Q_{th}(L)$ for each $L$.
%
In the MBL phase, the cluster structure is expected to be similar, independantly of system size, i.e. the average cluster length does not change with $L$. Therefore, as proven in appendix \ref{sec:scaling modularity}, the scaling of the modularity is given by:
\begin{equation}
\label{scaling_mod}
    Q(L)=q-\frac{a}{L},
\end{equation}
%
and therefore we choose:
\begin{equation}
    Q_{th}(L)=\alpha\left(1-\frac{a_{W=6}}{L}\right),
\end{equation}
where $\alpha \in [0,1]$ and $a_{W=6}$ is the coefficient fitted for $W=6$, the maximum disorder strength considered in this section, located deep into the MBL phase, where therefore the scaling given by Eq. \eqref{scaling_mod} is valid.
%
In the main text, we present results for $\alpha=0.3$, since empirically it has been found that good partitions usually have a modularity greater than 0.3 \cite{invention_modularity}. We show in Appendix \ref{sec:thresholds}  that the scaling collapse is not sensible to the choice of this coefficient.
%
The rationale for this choice goes as follow: since the modularity can never exceed the value of one, we expect the maximum possible disorder-averaged modularity for system size $L$ to be given by $(1-a_{W=6}/L)$. Taking a fraction of this value should yield a threshold in which finite size effects are well accounted for. 
%
Of course we need to choose $\alpha$ such that the modularity of almost all eigenstates deep in the ergodic (resp. MBL) phase is below (resp. above) $Q_{th}(L)$.
%
After focussing on the average cluster size, we will now investigate the structure of individual eigenstates using the clustering algorithms. 

